Incentives in Dominant Resource Fair Allocation under Dynamic Demands

Every computer system -- from schedulers in clouds (e.g. Amazon) to computer networks to operating systems -- performs resource allocation across system users. The defacto allocation policies are max-min fairness (MMF) for single resources and dominant resource fairness (DRF) for multiple resources which guarantee properties like incentive compatibility, envy-freeness, and Pareto efficiency, assuming user demands are static (time-independent). However, in real-world systems, user demands are dynamic, i.e. time-dependant. As a result, there is now a fundamental mismatch between the goals of computer systems and the properties enabled by classic resource allocation policies. We aim to bridge this mismatch. When demands are dynamic, instant-by-instant MMF can be extremely unfair over longer periods of time, i.e. lead to unbalanced user allocations as previous allocations have no effect in the present. We consider a natural generalization of MMF and DRF for multiple resources and users with dynamic demands: this algorithm ensures that user allocations are as max-min fair as possible up to any time instant, given past allocations. This dynamic mechanism remains Pareto optimal and envy-free, but not incentive compatible. However, our results show that the possible increase in utility by misreporting is bounded and, since this can lead to significant decrease in overall useful allocation, this suggests that it is not a useful strategy. Our main result is to show that our dynamic DRF algorithm is $(1+\rho)$-incentive compatible, where $\rho$ quantifies the relative importance of a resource for different users; we show that this factor is tight even with only two resources. We also present a $3/2$ upper bound and a $\sqrt 2$ lower bound for incentive compatibility when there is only one resource. We also offer extensions for the case when users are weighted to prioritize them differently.

==> ropeNetGeneration.tex <==
\begin{figure}[t] \centering
	%\begin{overpic}[width=1.0\linewidth,tics=10]{diansour_ropeNetGeneration_low}%,grid
    %\begin{overpic}[width=1.0\linewidth,tics=10]{diansour_ropeNetGeneration_high}%,grid
	%\end{overpic}
	\begin{overpic}[width=1.0\linewidth,tics=10]{mechpart_ropeNetInitialization}%,grid
    %\begin{overpic}[width=1.0\linewidth,tics=10]{mechpart_ropeNetGeneration_low}%,grid
    %\begin{overpic}[width=1.0\linewidth,tics=10]{mechpart_ropeNetGeneration_high}%,grid
    \put(8,-2){\small (a)}
    \put(40,-2){\small (b)}
    \put(68,-2){\small (c)}
    \put(89,-2){\small (d)}
	\end{overpic}
    \caption{
    The workflow of the rope net generation. (a) The cross-field aligned with the directions of the key loops (plotted by green circles). (b) The field-guided geodesic curves (plotted by various colors) traced from both two sides of the key loops (colored the same as their curves). (c) We obtain the nodes (red dots) and the curve edges (colored by various colors) between them to compose the rope net by solving a mixed-integer optimization. (d) To guarantee 4-degree connectivity for the nodes on the ending loops, we use a simple linking operation to connect them with random sampling points through Dijkstra shortest paths on the surface model. The obtained curves and the nodes compose the rope net.
    }
    \label{fig:ropeNetGeneration}
    \vspace{-7pt}
\end{figure}

